Evaluating the Morphosyntactic Well-formedness of Generated Texts

Text generation systems are ubiquitous in natural language processing applications. However, evaluation of these systems remains a challenge, especially in multilingual settings. In this paper, we propose L'AMBRE -- a metric to evaluate the morphosyntactic well-formedness of text using its dependency parse and morphosyntactic rules of the language. We present a way to automatically extract various rules governing morphosyntax directly from dependency treebanks. To tackle the noisy outputs from text generation systems, we propose a simple methodology to train robust parsers. We show the effectiveness of our metric on the task of machine translation through a diachronic study of systems translating into morphologically-rich languages.

==> images/diachronicplots.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
wmt & agr-conj-NOUN-NOUN:Case & agr-det-DET-NOUN:Gender & agr-flat@name-PROPN-PROPN:Number & agr-mod-ADJ-NOUN:Case & agr-mod-VERB-NOUN:Case & agr-mod-VERB-NOUN:Gender & agr-mod-VERB-NOUN:Number & agr-subj-NOUN-VERB:Gender & agr-subj-NOUN-VERB:Number & agr-subj-PRON-VERB:Person & agr-subj@pass-NOUN-VERB:Number & args-comp:obj-NOUN-VERB:depd:Case & args-comp:obj@x-VERB-ADJ:depd:VerbForm & args-comp:obj@x-VERB-VERB:depd:VerbForm & args-subj-NOUN-AUX:depd:Case & args-subj-NOUN-VERB:depd:Case & args-subj@pass-NOUN-AUX:depd:Case & args-udep-PRON-VERB:depd:Case & args-udep-VERB-NOUN:depd:VerbForm\\ 
'14 & 0.7789 & 0.9894 & 0.9974 & 0.9258 & 0.8244 & 0.9050 & 0.8525 & 0.9202 & 0.8719 & 0.9930 & 0.8592 & 0.9522 & 1.0000 & 1.0000 & 0.9521 & 0.9389 & 0.8909 & 0.8684 & 1.0000 \\ 
'15 & 0.7760 & 0.9861 & 1.0000 & 0.9123 & 0.8364 & 0.9041 & 0.8628 & 0.9085 & 0.8584 & 0.9884 & 0.8110 & 0.9522 & 1.0000 & 1.0000 & 0.9201 & 0.9275 & 0.9006 & 0.9028 & 1.0000 \\ 
'16 & 0.8088 & 0.9906 & 1.0000 & 0.9405 & 0.8392 & 0.9199 & 0.8779 & 0.9252 & 0.8700 & 0.9902 & 0.8521 & 0.9684 & 1.0000 & 1.0000 & 0.9451 & 0.9232 & 0.8889 & 0.9221 & 1.0000 \\ 
'17 & 0.8848 & 0.9900 & 1.0000 & 0.9714 & 0.9345 & 0.9300 & 0.9500 & 0.9670 & 0.9275 & 0.9972 & 0.9241 & 0.9804 & 1.0000 & 1.0000 & 0.9556 & 0.9364 & 0.8900 & 0.9259 & 1.0000 \\ 
'18 & 0.8962 & 0.9930 & 1.0000 & 0.9745 & 0.9332 & 0.9336 & 0.9470 & 0.9800 & 0.9378 & 0.9955 & 0.9367 & 0.9840 & 1.0000 & 1.0000 & 0.9619 & 0.9398 & 0.8846 & 0.9272 & 1.0000 \\ 
'19 & 0.8636 & 0.9928 & 1.0000 & 0.9758 & 0.9268 & 0.9424 & 0.9423 & 0.9718 & 0.9362 & 0.9972 & 0.9315 & 0.9873 & 1.0000 & 1.0000 & 0.9749 & 0.9386 & 0.9032 & 0.8734 & 1.0000 \\ 
}\diachronicdata

\begin{figure*}[t]
\centering
\begin{tabular}{m{4.5cm}m{4.5cm}m{4.5cm}}
\begin{tabular}{c}
\tikplotmiddle{agr-mod-VERB-NOUN:Number}{(a) {$r_{agree}(\mathtt{Verb,Noun,mod})\!\rightarrow\mathtt{Number}$}}\\
\tikplotshort{agr-mod-VERB-NOUN:Gender}{(d) $r_{agree}(\mathtt{Verb,Noun,mod})\!\rightarrow\!\mathtt{Gender}$}\\
\tikplotshort{args-comp:obj-NOUN-VERB:depd:Case}{(g) $r_{as}(\mathtt{N,V,comp\!:\!obj})\!\rightarrow\!\mathtt{N}_{\mathtt{Case}}\mathtt{=Acc}$}\\
\tikplotshort{args-subj-NOUN-AUX:depd:Case}{(h) $r_{as}(\mathtt{N,Aux,subj})\!\rightarrow\!\mathtt{N}_{\mathtt{Case}}\mathtt{=Nom}$}\\
\end{tabular}
&
\begin{tabular}{c}
\tikplot{agr-conj-NOUN-NOUN:Case}{(b) $r_{agree}(\mathtt{Noun,Noun,conj})\!\rightarrow\!\mathtt{Case}$}\\
\tikplotmiddle{agr-mod-ADJ-NOUN:Case}{(e) $r_{agree}(\mathtt{Adj,Noun,mod})\!\rightarrow\!\mathtt{Case}$}\\
\tikplotmiddle{args-subj@pass-NOUN-AUX:depd:Case}{(i) $r_{as}(\mathtt{N,Aux,subj@pass})\!\!\rightarrow\!\!\mathtt{N}_{\mathtt{Case}}\mathtt{=Nom}$}\\
%\tikplotshort{}{$r_{agree}(\mathtt{Adj,Noun,mod})\!\rightarrow\!\mathtt{Case}$}\\
\end{tabular}
&
\begin{tabular}{c}
\tikplot{agr-mod-VERB-NOUN:Case}{(c) $r_{agree}(\mathtt{Verb,Noun,mod})\!\rightarrow\!\mathtt{Case}$}
\\
\tikplotshort{agr-subj-NOUN-VERB:Gender}{(f) $r_{agree}(\mathtt{Noun,Verb,subj})\!\rightarrow\!\mathtt{Gender}$}
\\
\tikplotmiddle{args-udep-PRON-VERB:depd:Case}{(j) $r_{as}(\mathtt{Pron,V,udep})\!\!\rightarrow\!\!\mathtt{Pron}_{\mathtt{Case}}\!=\!\mathtt{Gen,\!Ins}$}\\
\\
\end{tabular}
\end{tabular}
% \vspace{-2em}
\caption{Diachronic analysis of select agreement ($r_{agree}$) and argument structure ($r_{as}$) rules in Russian WMT. We report the \textit{median} fluency score for each WMT year. WMT systems have been consistently improving on their fluency, but some phenomena are still challenging, such as handling agreement across conjuncted nouns (b) or the use of proper case for passive constructions (i) or for oblique objects (j).}
\label{fig:diachronic_results_rules_full}
\end{figure*}



==> images/gec_examples.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}r@{ \ }p{0.9\columnwidth}@{}}
    \toprule
    %\multicolumn{2}{l}{\small \textbf{German}} \\
    \small S: & \small Vielleicht verdienen Ärzte {\color{red}\textbf{ihre}} {\color{red}\textbf{aktuelle}} Gehalt . \\
    \small A: & \small{3 4$\ \mid \ $\textsc{R:Det:Form}$\ \mid \ $ihr} \\
    \small A: & \small{4 5$\ \mid \ $\textsc{R:Adj:Form}$\ \mid \ $aktuelles} \\
    \small T: & \small Vielleicht verdienen Ärzte \underline{ihr} \underline{aktuelles} Gehalt . \\
    %\midrule
    %\multicolumn{2}{l}{\small \textbf{Russian}} \\
    %\small S: & \small \foreignlanguage{russian}{Текст включает в себя {\color{red}этимология} и {\color{red}история} употребления слова .} \\
    %\small A: & \small{4 5$\ \mid \ $\textsc{Noun:Case}$\ \mid \ $\foreignlanguage{russian}{этимологию}} \\
    %\small A: &\small{6 7$\ \mid \ $\textsc{Noun:Case}$\ \mid \ $\foreignlanguage{russian}{историю}} \\
    %\small T: & \small \foreignlanguage{russian}{Текст включает в себя \underline{этимологию} и \underline{историю} употребления слова .} \\
    \bottomrule
    \end{tabular}
    %\caption{Example sentences from the German and Russian GEC datasets. Incorrect words are colored {\color{red}red}, with correct forms \underline{underlined}. Applying the annotations (A) to the source sentence (S) produces the well-formed target sentence (T).}
    \caption{Example sentence from the German GEC dataset. Incorrect words are colored {\color{red}\textbf{red}}, with correct forms \underline{underlined}. Applying the annotations (A) to the source sentence (S) produces the well-formed target sentence (T).}
    \label{tab:gec_dataset_examples}
    \vspace{-1em}
\end{table}

==> images/gec_metric_comparison_dev.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}lc@{ \ }c@{ \ }c@{}}
    \toprule
    Contrast & \mname{} & GBM & PPL \\
    \midrule
    \multicolumn{4}{l}{\textbf{German}} \\
    \midrule
    (src, tgt) & 0.29 (0.27) & \underline{0.62} & \textbf{0.96} \\
    (src, morph-corrected) & 0.32 (0.29) &\underline{0.34} & \textbf{0.74} \\
    (src, rest-corrected) & 0.18 (0.18) & \underline{0.58} & \textbf{0.94} \\
    (morph-corrected, tgt) & 0.19 (0.18) & \underline{0.61} & \textbf{0.97} \\
    (rest-corrected, tgt) & 0.43 (0.38) & \underline{0.46} & \textbf{0.96} \\
    \midrule
    \multicolumn{4}{l}{\textbf{Russian}} \\
    \midrule
    (src, tgt) & 0.22 (0.20) & \underline{0.40} & \textbf{0.90} \\
    (src, morph-corrected) & \underline{0.25} (0.22) & 0.14 & \textbf{0.69} \\
    (src, rest-corrected) & 0.13 (0.12) & \underline{0.42} & \textbf{0.86} \\
    (morph-corrected, tgt) & 0.18 (0.16) & \underline{0.48} & \textbf{0.92} \\
    (rest-corrected, tgt) & \underline{0.40} (0.34) & 0.21 & \textbf{0.95} \\
    \bottomrule
    \end{tabular}
    \caption{Accuracy results for \mname{}, grammaticality-based metric (GBM), and perplexity (PPL) on various contrastive acceptability judgments on German and Russian GEC (\textit{dev} splits). Best score is in \textbf{bold}, and the second best score is \underline{underlined}. Numbers in parantheses are obtained by using original stanza parsers instead of the proposed robust parsers.}
    \label{tab:gec_contrast}
\end{table}

==> images/lambre_scoring_example.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}c@{}}
         \toprule
    \begin{tabular}{@{}l@{ \ }l@{ \ }l@{ \ }l@{ \ }l@{}}
    %\toprule
        \textsc{pron} & \textsc{aux} & \textsc{adj} & \textsc{noun} & \textsc{verb} \\
        (*) Ich & werd\textcolor{red}{\textbf{en}} & lange\textcolor{red}{\textbf{n}} & B\"{u}cher & lesen \\
        \textsc{nom.1sg} & \textsc{1\textcolor{red}{\textbf{pl}}} & \textsc{\textcolor{red}{\textbf{dat}}.pl} & \textsc{acc.pl} & \textsc{ptcp}\\
    \end{tabular}\\
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c}
    \midrule
    \textbf{Rules} & \textbf{Score} \\
    \midrule
    \multicolumn{2}{l}{\textbf{Agreement}}\\
    $r_{\textit{agree}}(\mathtt{ADJ},\mathtt{NOUN},\mathtt{mod})\rightarrow \mathtt{Number}$ & 1 \\
    $r_{\textit{agree}}(\mathtt{ADJ},\mathtt{NOUN},\mathtt{mod})\rightarrow \mathtt{Case}$ & 0 \\
    $r_{\textit{agree}}(\mathtt{ADJ},\mathtt{NOUN},\mathtt{mod})\rightarrow \mathtt{Gender}$ & 1 \\
    $r_{\textit{agree}}(\mathtt{PRON},\mathtt{AUX},\mathtt{subj})\rightarrow \mathtt{Number}$ & 0 \\
    $r_{\textit{agree}}(\mathtt{PRON},\mathtt{AUX},\mathtt{subj})\rightarrow \mathtt{Person}$ & 1 \\
    \midrule
    \multicolumn{2}{l}{\textbf{Case Assignment}}\\
    $r_{\textit{as}}(\mathtt{NOUN},\mathtt{VERB},\mathtt{comp}\mathtt{:}\mathtt{obj})\rightarrow \mathtt{Case}_{\mathtt{NOUN}}$=$\mathtt{Acc}$ & 1 \\
    % $r_{\textit{as}}(\textit{comp:aux},\texttt{VERB},\texttt{AUX})\rightarrow \textit{VerbForm}_{\texttt{Verb}}$=$\text{Inf,Part}$ & 1.0 (Inf) \\
    $r_{\textit{as}}(\mathtt{PRON},\mathtt{AUX},\mathtt{subj})\rightarrow \mathtt{Case}_{\mathtt{PRON}}$=$\mathtt{Nom}$ & 1 \\
    \midrule
    \multicolumn{1}{r|}{\mname{} agreement score} & 0.6 \\
    \multicolumn{1}{r|}{\mname{} case assignment score} & 1.0 \\
    \multicolumn{1}{r|}{\mname{} overall score} & 0.71 \\
    \end{tabular}}\\
    \bottomrule
    \end{tabular}
    \caption{Scoring on agreement and case assignment rules for the A.2 example of Figure~\ref{fig:overview}. We give a score of 1 for each successful application of the rule, 0 otherwise.\ap{Some repetition with Figure~\ref{fig:overview}, make it inline.} }
    \label{tab:scoring_example}
    \vspace{-1em}
\end{table}

==> images/morphology_noise_dist.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/noise.png}
    \caption{Distribution of morphological features altered for Czech (ces), Greek (ell), Russian (rus), Spanish (spa), Turkish (tur).}
    \label{fig:noise_morphology}
\end{figure}

==> images/ppl_ud_results.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{@{}l|c|c}
    \toprule
    Treebank & Acc\textsubscript{ppl} & Acc\textsubscript{\mname{}} \\
    \midrule
    German-HDT & 95.77 & 99.53 (99.93*) \\
    Russian-SynTagRus & 97.93 & 99.24 (99.95*) \\ 
    \bottomrule
    \end{tabular}
    \caption{Comparison of perplexity and \mname{} on UD dev splits. Numbers in parentheses use gold parse and morphological tags.}
    \label{tab:ud_perplexity}
\end{table}

==> images/wmtfig.tex <==

\input{images/wmt}

\begin{figure}[t]
\centering
\begin{tabular}{p{3.8cm}p{3.8cm}}
\wmtplot{\csdata}{\csavg}{Czech}{.85} & 
\wmtplot{\rudata}{\ruavg}{Russian}{.85}\\
\wmtplot{\dedata}{\deavg}{German}{.85}&
\wmtplot{\fidata}{\fiavg}{Finnish}{.75} \\
\wmtplot{\trdata}{\travg}{Turkish}{.93} & \\
\multicolumn{2}{c}{\small $\blacksquare$: systems average \ \ \textcolor{red}{$\circ$}: system \ \ $\bullet$: reference}\\
\end{tabular}
    \caption{A diachronic study of grammatical well-formedness of WMT English$\rightarrow$X systems' outputs. The systems in general are becoming more fluent with very passing year. In the last two years the best systems produce as well-formed outputs as the reference translations.} %\ap{should we report median or mean score?}}
    \label{fig:diachronic_results_full}
    \vspace{-1em}
\end{figure}
